Generative Deep Learning Techniques for Password Generation

Password guessing approaches via deep learning have recently been investigated with significant breakthroughs in their ability to generate novel, realistic password candidates. In the present work we study a broad collection of deep learning and probabilistic based models in the light of password guessing: attention-based deep neural networks, autoencoding mechanisms and generative adversarial networks. We provide novel generative deep-learning models in terms of variational autoencoders exhibiting state-of-art sampling performance, yielding additional latent-space features such as interpolations and targeted sampling. Lastly, we perform a thorough empirical analysis in a unified controlled framework over well-known datasets (RockYou, LinkedIn, Youku, Zomato, Pwnd). Our results not only identify the most promising schemes driven by deep neural networks, but also illustrate the strengths of each approach in terms of generation variability and sample uniqueness.

==> data_i/gpt2_pretrained.tex <==
patjay98 rolly1230 rggp2201 preswad42 papa9020 shard98 sevdeni panopis15 rolexnt remel03 nswedl1 paul2435 segredo22 odboy24 s62206 satine90 pikacheese plaa789 renny1706 poogleboo s8323410j seanbray pol1o00 otterbeer sahilak44 oavkifry shvnjlm sexyblues6 phi714 roxy6995 scottdyan shanesmommy sammykane1 s9274879z penfish302 piggygirl18 qhotrbo1qhotrod rockyoudjv pumas212 prince4juju rick5457 p4ls4k9 sexpuss18 presley86 sfr321 one18only paul2117 shicarlos ray1311 s331942 bmj522 chinaakai aperren20 c0308r apinya06 ashroy30 cj1013 ballmax917 bujies09 coolcess11 ba9b4y4j7l9i9 apsolove47 bong000 cinder07 chris_rox cheyanne37 babyangie7 crl30100 bobbvb changss corykyle2 arsalee babyt923 caprix bman408 buck0821 carlouse biarte benyo2214 boom0823 cre9inja3 biac9525 catbalss. cali918 bffandm d3m0n8 asha104 bidou123 bokbet ceritaluna chelsie1020 azul1141 bigback23 cmp8302 ca12179 chompocz cap123456789 carabito c1w2e3r4m5 beccalo


==> data_i/gpt2_scratch.tex <==
tatoking ternex8 starchef sneakywoo yannik1 westlife01 sll1977 yeunsumari uriah3224 theklonde teamoo14 tg29803 sweet487 thanny2 switchi sushigrl2 woodleck30 tsweetpea86 volks777 tati2527 smile0420 woodsy25 thetate! tgbtgar trav08 wut66ger wynokk sykis xpiloticox swedish wtk5246 vald154 test1829 tele7124 wings69 trisht zf4750 traviesajoan tickshade tlcb24 suse thereisley7 spud90 tif14 walnutgate um127 uganda9 toppops yohanjoanna virz238 susijust tslitty tonys19 tenary welkom spanne 1girl vjfempro tonyh2 sygda umhs2save tibhall xeldel1 terunea vicdar23 whitemaylor tyric? vistar4 unme91 wynnerly33 tywank57 tamash syldia swooches1 symbian timmons29 sonic831 yoeltz vfjmonair tymecca taik922 soccer621 tyjepoun twista tongshan83 xiji2323 surabi sm104139 silva001 vwchie xin123 tjasa urapoll vmlkfv9 stjeff10 woochle79 suajai2009 sparman04 tifo1979 sofirenny


==> data_ii/most_common_passwords.tex <==

\iffalse
GPT2S pwnd
  14601 2010
  14452 love
  14120 1234
  11486 2000
  10189 2009
   9969 2008
   9949 12345
   9914 2011
   8799 2007
   8148 1992


GPT2S rockyou
  25404 love
  13691 mrs.
  11300 baby
  11282 sexy
   8393 girl
   8008 angel
   7586 1992
   7094 1993
   7091 1994
   7066 2007

GPT2F rockyou
   1570 ilove
   1338 love
   1099 baby
    986 iluv
    692 sexy
    675 pink
    621 memyself
    541 caoimhe
    524 cintaku
    483 jess


GPT2F pwnd
  15932 1234
  15184 2010
  14734 love
  12584 2000
  11349 2009
  11180 2008
  11164 12345
  10524 2011
   9278 2007
   8595 1987
   
VAE rockyou
    1192 leslie
    1111 yankee
    1092 kirsty
    986 jeremy
    956 claudia
    940 gangsta
    922 violet
    921 andrei
    918 jennifer
    904 natalie
    
    
VAE pwnd
    46 MARIA
    41 hilton
    38 SEXY
    38 4678
    37 NATA
    36 ALEX
    34 JOSE
    34 BABY
    30 MAMA
    30 ANGEL
    29 4ever
    29 1myspace
    28 STAR
    28 PAPA
    28 2myspace
    27 ROSE
    27 JAMES
    25 margate
    24 aleksey
    24 MARK
    
    
PassGAN rockyou
    985846 123456
     323478 12345
     162398 123456789
      94956 1234567
      75377 12345678
      21160 angela
      21044 angels
      15947 angel1
      15751 buster
      14961 128456

\fi


==> sections_i/conclusion.tex <==
Considering the reported results and model performance it appears that deep learning models based on attention mechanisms (GPT2 and Transformers) and representation models (VAE) are a very promising direction for further investigation. In comparison to adversarial schemes autoencoding as well as attention-based models performed nearly twice as good in terms of generating and guessing new meaningful passwords. It should be noted that for smaller numbers of generated passwords the performance difference is less obvious (i.e. up to $10^6$ generated samples). Moreover, our PassGAN models seem to outperform the results outlined in \cite{Hitaj2017}.

However, a possible reason for the poorer GAN performance in comparison to VAE, GPT2 seems to stem from, on one hand, the lack of structural awareness (i.e. discovering the password patterns via latent representations), on the other hand, the training instability that is often reported for adversarial optimization.

Some future and upcoming work directions would be, e.g., the following:
\begin{itemize}
	\item A natural next step is deploying and adapting the models to further datasets (the initial use of "rockyou" was motivated by \cite{Hitaj2017} as being a standard benchmark that strikes balance between training time and data complexity).
	\item A future detailed comparison of deep learning models against other statistical methods (used throughout the community) is needed in order to justify the above methods as useful tools in the subject.
	\item It is reasonable to investigate other methods of shaping the latent space of VAE and adding additional structure to the model (attention, semi-supervised methods, discrete latent representations, etc).
	\item An investigation of sampling techniques towards better password generation.
	\item The above steps would require further adaptation of the proposed deep learning models, e.g. by fusing some statistical preprocessing and introducing further data embeddings based on suitably obtained meta-data and statistical evaluation. In other words, we believe that attempting to bridge solutions based on "pure" statistical methods with appropriate state-of-art deep neural networks is a promising research direction to be further pursued.
\end{itemize}

==> sections_i/gan.tex <==
A central idea of adversarial methods is the construction of generative models by game-theoretic means: a "generator" neural network produces data samples, whereas a "discriminator" neural network simultaneously attempts to discern between the real and artificially produced (by the generator) samples. The training of such a system consists in optimizing the performance of both the generator and discriminator (usually, via types of suitably chosen gradient descents and additional regularization). Since the relevant technical aspects of GANs were already discussed in previous LILY reports we omit the basic details; we also once more refer to \cite{Goodfellow2014}, \cite{Arjovsky2017}, \cite{Gulrajani2017}.

Concerning password guessing and generation our starting point is the well-known PassGAN model proposed in \cite{Hitaj2017} and also studied in previous LILY reports. The original PassGAN defines a discriminator and generator in terms of residual networks \cite{Zagoruyko2016} - these are assembled from the so-called residual blocks (e.g. a stack of convolutional neural networks followed by a batch-normalization \cite{Ioffe2015}). A specific feature here is that the input partially bypasses the residual block (shortcutting) and is added to the output of the residual block - the aim is to diminish the effect of vanishing gradients and introduce a form of "memory" across the residual network.


In our setup, we essentially utilize the PassGAN as a standard benchmark. The generator/discrimintor are defined as resdiual neural networks consisting of 6 standard residual blocks followed by a linear projection/softmax function, respectively. Each of the standard residual blocks consists of 2 convolutional layers (with kernel-size 3, stride 1, no dilation) followed by a batch-normalization layer. The generator's latent space (i.e. the input space) is set to 256 inspired by \cite{Hitaj2017}.

\subsection{Training}
The PassGAN training was based on some state-of-art practices such as Wasserstein GAN and gradient clipping (cf. \cite{Arjovsky2017}), as well as gradient penalty regularization (cf. \cite{Gulrajani2017}). We mostly used a batch-size of 256, a gradient-penalty-hyperparameter $\lambda$ set to 10 and 10 discriminator iterations per generator step. The preferred gradient descent was based on ADAM with an initial learning rate of $\sim 10^{-4}$ and beta (momentum) parameters $0.5, 0.9$; a fixed-interval annealing with an iteration step of $\sim 10^6$ was also used.






==> sections_i/introduction.tex <==
Deep learning models have recently shown remarkable performance concerning text classification and text generation. Major advancements in the field have been fueled by the development in several central directions such as:

\begin{enumerate}
	\item \textbf{The \textit{attention} mechanisms}. Considering a token (word, letter, sentence) within a textual environment, the idea is to develop a flexible notion of \textit{context} that connects the given token with other pieces of the textual environment. Intuitively, this allows the learning model to better grasp the textual structure (e.g. grammar, semantic meaning, word structure, etc), thus leading to eventual improvements in terms of text classification/generation/interpretability. Among others, well-known attention-based examples are given by BERT, ELMO, GPT and various further types of Transformers.
	
	\item \textbf{Model architectures and representation capabilities}. Remarkable progress has been made in designing more flexible deep learning structures (CNN-based ResNets and Wide-Resnets, recurrent NNs, adversarial models, etc). The success of these deep neural networks can to a large extent be attributed to their \textit{representation capability}, i.e. they create an appropriate transformation of the data (e.g. compression or a sort of "semantic meaning" extraction) that renders the data easier to handle and solve a given problem. In this regard a central class of deep learning models is given by the so-called \textit{\textbf{autoencoders}} whose goal is not only to create a meaningful and useful data representation/transformation (Encoding) but also to be able to go back and reconstruct the initial data from the representation (Decoding). An upshot is that one could \textit{generate new data} by sampling points in the representation space and then decoding back.
	
	\item \textbf{Advanced training procedures}. The above tools would not be as effiecient, had not it been for the corresponding methods to select (train) the parameters and weights of the neural networks. Among others these include appropriate momentum and annealing-driven stochastic gradient descents, Wasserstein regularization and variational approaches.
\end{enumerate}

On the other hand, considering password guessing problems, some popular frameworks (HashCat, John-The-Ripper, etc) as well as a large body of state-of-art research suggest that advanced deep learning methodologies are still to be further explored. Ideally, one would attempt to design more efficient password-guessing models aided by neural networks and cutting-edge practices. In the following we present our initial steps in this exploration where the focus was laid on three architecture types: GANs, variational autoencoders and transformers.



==> sections_i/representation_learning.tex <==
Many real world task as well as machine learning tasks can be solved very difficult or very easy depending on how the information is represented. Let us take for example the task of dividing the number 180 by 2. The task is straight forward using the Arabic numeral system. Now, we pose the same problem but we use the Roman numeral system to represent the numbers. In this case the task is dividing CLXXX by II. Using the Roman numeral system the task seems much more difficult for a modern educated person.

Representation learning is interesting because it provides one particular way to perform unsupervised learning. Unsupervised deep learning algorithms have a main training objective but also learn representations as side product. Naturally arises the question: \textit{What makes one representation better than another?} In the context of machine learning a representation $\mathbf{z}$ is good if it makes the subsequent task easy to solve. One hypothesis out there is that the best representation is the one in which each of the features within the representation corresponds to the underlying factors or causes that generated the observed data. In ideal case each of the features or directions in the features space corresponds to different causes of the data. This kind of representation disentangles the underlying generative factors and they are called \textit{disentangled} representation. There is a large body of deep representation learning research focused on obtaining disentangled representation.

\textit{Why representation learning is important in password guessing setting?} There has been extensive research on text-password attacks and how people are choosing passwords. Human chosen passwords are not uniformly distributed in the space of passwords (all possible strings). But the user tend to pick passwords that are easy to remember or have some personal meaning. Also every web services has different policies about password construction (length, number of symbol, capital letters and etc.) Therefore, one can conclude that there are different latent factors in constructing a password. If we are able to learn these different factors, it will be possible to generate passwords that are from the same distribution as the human generated passwords.


\subsection{Variational Auto Encoder}
\label{ssec:vae}

The Variational Auto Encoder (VAE) \cite{kingma2013auto} is generative model that comprises of two main components: i) \textit{encoder} and ii) \textit{decoder}. The encoder is stochastic function $\phi: \mathbf{X} \rightarrow\mathbf{Z}$ that maps the input space (passwords) $\mathbf{X}$ to the latent space $\mathbf{Z}$. The decoder is deterministic function that maps a code from the latent space to the input space $\theta: \mathbf{X} \rightarrow\mathbf{X}$. The model is trained by maximizing the log likelihood

\begin{equation}
  \mathcal{L}(\mathbf{\theta, \phi, x^{(i)}})=-D_{KL}(q_{\phi}(\mathbf{z}|\mathbf{x}^{(i)})||p_{\theta}(\mathbf{z}))+\mathbb{E}_{q_{\phi}(\mathbf{z}|\mathbf{x}^{(i)})}\left[\log{p_{\theta}(\mathbf{x}^{(i)}|\mathbf{z})}\right].
\label{eq:vae_loss}
\end{equation}

Training the model is done by minimizing the loss function Eq. (\ref{eq:vae_loss}). The model learns to reconstruct the password $\mathbf{x}$ given to the input by first mapping the password to a distribution of latent codes $p_{\psi}(\mathbf{z}|\mathbf{x})$ than we sample from the posterior distribution and we pass the latent code $\mathbf{z}$ to the decoder $p_{\theta}(\mathbf{x}^{(i)}|\mathbf{z})$. During training a strong prior $p(\mathbf{z})$ is imposed on the learned latent code distribution, this is done so later we can easy sample from them and generate new passwords.In this way we learn a latent space

The latent space learned by the encoder imposes a geometric connections among latent points that have some semantic similarity in the data space. As a result \textit{similar} points in the data space have latent representation that are close to each other. The notation of \textit{similarity} depends on the modeled data, in the case of password generation it can be based on the structure of the password, the common substring, etc.

\textbf{Similarity in latent space.} In Table (\ref{tab:latent_space_similarity}) are presentend samples with latent representations close to the latent representation of the password \verb|veronica2296|.

\begin{table}[h]
\centering
\begin{tabular}{lllll}
\verb|veronica2286|  & \verb|veronica296|   & \verb|verogani2297|  & \verb|veronica2229| & \verb|veroicata22U| \\
\verb|veronica22U6|  & \verb|veronic22259|  & \verb|veroinca2297|  & \verb|verolica2296| & \verb|verotEic2246| \\
\verb|verogama2296|  & \verb|veronica2269|  & \verb|veronica22_9| & \verb|veronica239|  & \verb|verolica2298| \\
\verb|veroga_a2986| & \verb|veronic2205|   & \verb|veronaxa2269|  & \verb|veronico2259| & \verb|verolicat269| \\
\verb|verosgaj2!98|  & \verb|vertinac2219|  & \verb|veronica249|   & \verb|verincia22T6| & \verb|veronema2205| \\
\verb|veroina22_6|  & \verb|verozica22_|  & \verb|veroszi2246|   & \verb|veronkea2295| & \verb|verolica2295| \\
\verb|veroneza2269|  & \verb|veron_ma2295| & \verb|verogaxa2299|  & \verb|veronica4298| & \verb|verote5a229D| \\
\verb|veronica20g6|  & \verb|verogala285|   & \verb|verozoca24_7| & \verb|veronic22#6| & \verb|veronoca28/5| \\
\verb|veronico23D|   & \verb|veronema2276|  & \verb|veronica2296|  & \verb|veronican298| & \verb|veronicas25|  \\
\verb|vroricak229|   & \verb|verongic2279|  & \verb|vegaroaka269|  & \verb|veronica2896| & \verb|vetRonic225|  \\
\end{tabular}
\caption{Samples with latent representation close to \textit{veronica2296} latent representation.}
\label{tab:latent_space_similarity}
\end{table}

\textbf{Conditional password generation.} Having latent representation for each password allows us to also do conditional generation. Let \textit{***love***} be a template password. The '*' symbol it is a placeholder for any character defined in the vocabulary. We can condition our model to generate passwords that contain the word `love` in the middle, with three random characters as prefix and suffix. In Table (\ref{tab:conditional_generation}) are presented some conditionally generated samples.

\begin{table}[h]
\centering
\begin{tabular}{llll}
\verb|9alolove71u| & \verb|nublove85/9| & \verb|miblovenv11| & \verb|cetlovesder| \\
\verb|licloverrs9| & \verb|siclove00me| & \verb|riglover2k|  & \verb|biolove121|  \\
\verb|hicloven3ke| & \verb|failoveye4|  & \verb|n2ulovemswo| & \verb|inudlove12|  \\
\verb|lyaloveji8|  & \verb|gemloveso1|  & \verb|irolovesor|  & \verb|Vealover.v|  \\
\verb|ltelovejr*|  & \verb|vatlover10|  & \verb|mejlovey4u|  & \verb|sewalover79| \\
\end{tabular}
\caption{Conditional generation of passwords. We condition the generation on \textit{***love***}.}
\label{tab:conditional_generation}
\end{table}


\textbf{Interpolation between two passwords.} Another possibility with the VAE models is to do interpolation between two passwords. Let us assume we have the password $A$ and the password $B$. We use the encoder to obtain the latent representations $\mathbf{z}_A$ and $\mathbf{z}_B$ for $A$ and $B$ respectively. Next, we sample latent representations from the linear path former by $\mathbf{z}_A$ and $\mathbf{z}_B$ and using the decoder we obtain the corresponding passwords. The process of sampling new passwords in this way is called \textit{interpolation}. In Table (\ref{tab:interpolations}) are given some example interpolations. Each column in the table is an example interpolation. The top row is the password $A$ and the bottom row is the password $B$. In the middle are the passwords generated from the latent representations sampled form the linear path between $A$ and $B$

\begin{table}[h]
\centering
\begin{tabular}{llllll}

\verb|remington223| & \verb|pepegrillo16|  & \verb|newthanakorn|   & \verb|musikALE0991| & \verb|DIMAYUGAluna| & \verb|fressikarosa| \\
\verb|rtninton2131| & \verb|popegrillo16|  & \verb|nevwhanfaror|   & \verb|muwikO134902| & \verb|DIMAYUYAUMEM| & \verb|krezsickiess| \\
\verb|Atnitton2133| & \verb|petckrllole7|  & \verb|new_hanaqira|   & \verb|muwIE1250894| & \verb|DIMuYuYnuMAY| & \verb|kryesikarish| \\
\verb|ntn123to2131| & \verb|hoperillel62|  & \verb|newsafarhrig|   & \verb|memIE1284989| & \verb|GIMAYuYuuakH| & \verb|kynesiha2308| \\
\verb|rmnm2et21213| & \verb|agterillo652|  & \verb|18stahankoua|   & \verb|mTO130281948| & \verb|VUHuwuNAuMMe| & \verb|kynayiha2s09| \\
\verb|nnnmot121032| & \verb|ktanlilel657|  & \verb|18s7tafabano|   & \verb|K72636481934| & \verb|WHfluvusue85| & \verb|cynayoshi_09| \\
\verb|nnd231523465| & \verb|allininal505|  & \verb|129swokfaton|   & \verb|172639451658| & \verb|Tofluousuck9| & \verb|cy2ayueh2990| \\
\verb|ontit1321642| & \verb|allinllang08|  & \verb|1287tockokno|   & \verb|172639293483| & \verb|WofdmousuS86| & \verb|clyayosh1090| \\
\verb|andiew123456| & \verb|alliannan680|  & \verb|12960ocktint|   & \verb|172839481614| & \verb|moodmous6885| & \verb|clya23081099| \\
\verb|andrew123456| & \verb|allianna0685|  & \verb|1297bucktown|   & \verb|172839456123| & \verb|woodmouse598| & \verb|clya23081990| \\
\end{tabular}
\caption{Example interpolations. Each column is one interpolation where the top row is the start password $A$ and the last row is the end password $B$. In between are generated passwords.}
\label{tab:interpolations}
\end{table}



==> sections_i/results.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}
% \usepackage{arydshln}

A major goal of the present paper is to obtain an initial understanding of how capable the proposed models above are in terms of basic password guessing/generation. To this end we largely followed the benchmark strategy proposed in \cite{Hitaj2017} where PassGAN was evaluated. Similarly, we train our models on the well-known "rockyou" dataset where we set aside $10\%$ for validation and $10\%$ for testing purposes. As suggested in previous LILY reports and \cite{Hitaj2017}, after being trained we benchmark the model using the amount of passwords it is able to recover from the test set. Moreover, in contrast to \cite{Hitaj2017} we restrict to and generate sequences consisting of 12 characters (instead of 10).


In the above setup a detailed results' overview is avaiable in tables  \ref{tab:full-results}, \ref{tab:aggregated-results} and \ref{tab:aggregated-results-LinkedIn}. The training was conducted as specified for each particular model.


\subsection{Samples}
\textbf{PassGAN}:
\begin{verbatim}
cooljessy relora babybey1 icukyday sweetlove ohesas dwck15 eeblen 45058369
081012026 lovelleh3 love11 rhimata15 thumbap? iloveunk michle1 cuyeau15 marhela
talawow tarobal (ock yme stank8106 sprimadaj sascat08 332072 ajohs17 kjulya
asecow grel62 jesn12 muttin manken keggck putol17 <izgerR1 tinge06 97764582
kowiz myster  207878 wern02 teamyroo1 t0rye duliaw1 mel0107 #erist ghweet soggan
teams lamaw2 jap45 bl94164 pop15 RilTDOR coopie stert04 J<QnCeORz trucky sister00
19345 redena jabelle taggifgo alcjul 062199 IRELTDYR 123456 werdune9 wap456
cadfiraI lovelo coopy loleditot kengtt 1491464 100598 remily 260896 befler1
kentissa sarspoge1 davin13 25458504 hitmans10199 lupe75 dagassapio 1977som ad9656
00047213 hhaipet dorilair1 bushy15 leon16 1Macesd marwy1343 lotter_sag carssman11 czalisaya
belatofun scoopie21 abdiabuy biham4eva creegeg 76DIEGO phiookan12 bambigar
7839aj karenequiero jhayward aleeka corals10DO jentep marian68 weriter
pollopop21 htank05 marlloven joyshayle iversonluf abael35 rgas83100 steelnell1 jkrail javamme
deksu1 minimar jenne4754 119654c JAGUARD bonelfoolita charleyme! gmon24
\end{verbatim}

\textbf{Variational Auto-encoder:}
\begin{verbatim}
chivinic greenlegurl 099957294 191623556 829547522 337241 uke1428 612790904 eaweshay96
12934213 583705 Ashton666 matemaria aedhti COOKIES22 2008252n ILOVEDS12 tastynm_25
tme17110 karla4720 7odtlz 216585 kdtaly 1126943 057910911 Norris16 joesalu 2jt4haf
04yscgo! zyman2005 lightsc ystin317 689795 mividoggy kmw2002 susan98 krenuta10 ALIASD
055040760 divo311 bravel03 shuture3 ayanher2 2096fj 09189037401 740133833 nys1724
358879 ballo42 bocasta13 vhiempum 269428 3759543 mbvp1310 BAC1LAN 19912005 2005142513
5371rr june999 poony0129 0132car csabura707 atrogui 88021607528 patoss79
seran1 8528296 022335b ryleejoe2 sister2 DICEE27 zombirn99 namo1819 0774171177
biabel 25260302 bougee24 pricertamp1 0802741016 blackspek ati2006* bruce123
\end{verbatim}


\textbf{GPT2F:}
\begin{verbatim}
patjay98 rolly1230 rggp2201 preswad42 papa9020 shard98 sevdeni panopis15 rolexnt
remel03 nswedl1 paul2435 segredo22 odboy24 s62206 satine90 pikacheese plaa789 renny1706
poogleboo s8323410j seanbray pol1o00 otterbeer sahilak44 oavkifry shvnjlm sexyblues6
phi714 roxy6995 scottdyan shanesmommy sammykane1 s9274879z penfish302 piggygirl18
qhotrbo1qhotrod rockyoudjv pumas212 prince4juju rick5457 p4ls4k9 sexpuss18 presley86
sfr321 one18only paul2117 shicarlos ray1311 s331942 bmj522 chinaakai aperren20 c0308r
apinya06 ashroy30 cj1013 ballmax917 bujies09 coolcess11 ba9b4y4j7l9i9 apsolove47 bong000
cinder07 chris\_rox cheyanne37 babyangie7 crl30100 bobbvb changss corykyle2 arsalee
babyt923 caprix bman408 buck0821 carlouse biarte benyo2214 boom0823 cre9inja3 biac9525
catbalss. cali918 bffandm d3m0n8 asha104 bidou123 bokbet ceritaluna chelsie1020 azul1141
bigback23 cmp8302 ca12179 chompocz cap123456789 carabito c1w2e3r4m5 beccalo
\end{verbatim}


\textbf{GPT2S:}
\begin{verbatim}
tatoking ternex8 starchef sneakywoo yannik1 westlife01 sll1977 yeunsumari uriah3224
theklonde teamoo14 tg29803 sweet487 thanny2 switchi sushigrl2 woodleck30 tsweetpea86
volks777 tati2527 smile0420 woodsy25 thetate! tgbtgar trav08 wut66ger wynokk sykis
xpiloticox swedish wtk5246 vald154 test1829 tele7124 wings69 trisht zf4750 traviesajoan
tickshade tlcb24 suse thereisley7 spud90 tif14 walnutgate um127 uganda9 toppops
yohanjoanna virz238 susijust tslitty tonys19 tenary welkom spanne 1girl vjfempro
tonyh2 sygda umhs2save tibhall xeldel1 terunea vicdar23 whitemaylor tyric? vistar4
unme91 wynnerly33 tywank57 tamash syldia swooches1 symbian timmons29 sonic831 yoeltz
vfjmonair tymecca taik922 soccer621 tyjepoun twista tongshan83 xiji2323 surabi sparman04
tifo1979 sofirenny sm104139 silva001 vwchie xin123 tjasa urapoll vmlkfv9 stjeff10
woochle79 suajai2009
\end{verbatim}




\begin{table}
    \centering
    \begin{tabular}{l|l:l:l:l:l}
        & & & & &                      \\

        Model &
        \begin{tabular}[c]{@{}l@{}}Passwords\\Generated\end{tabular} &
        \begin{tabular}[c]{@{}l@{}}
            Unique\\Passwords
        \end{tabular} &
        \begin{tabular}[c]{@{}l@{}}
            Unique\\Passwords \%
        \end{tabular} &
        Matched &
        Matched \%  \\

        \toprule
        \multirow{7}{*}{\begin{tabular}[c]{@{}l@{}}
                            GPT2 - Finetuned\\(GPT2F)
        \end{tabular}}
        & $10^2$ & 100      & 100  & 1      & 0.00                       \\
        & $10^3$ & 1000     & 100  & 13     & 0.00                       \\
        & $10^4$ & 10000    & 100  & 123    & 0.01                      \\
        & $10^5$ & 99897    & 99.9 & 1157   & 0.09                      \\
        & $10^6$ & 992409   & 99.2 & 10884  & 0.84                      \\
        & $10^7$ & 9452453  & 94.5 & 87908  & 6.75                      \\
        & $10^8$ & 77193402 & 77.2 & 330990 & 25.42       \\

        \midrule
        \multirow{7}{*}{\begin{tabular}[c]{@{}l@{}}
                             GPT2 - Scratch\\(GPT2S)
        \end{tabular}}
        & $10^2$ & 100 & 100 & 1 & 0.00                      \\
        & $10^3$ & 1000 & 100 & 16 & 0.00                      \\
        & $10^4$ & 9984 & 99.8 & 143 & 0.01                      \\
        & $10^5$ & 99304 & 99.3 & 1698 & 0.13                      \\
        & $10^6$ & 940487 & 94.0 & 14661 & 1.13                      \\
        & $10^7$ & 8083531 & 80.8 & 93016 & 7.14                      \\
        & $10^8$ & 70582659 & 70.6 & 310931 & 23.87         \\
        & $10^9$ & 454070343 & 45.4 & 531666 & 40.82         \\

        \midrule
        \multirow{7}{*}{PassGAN}
        & $10^2$ & 97 & 97 & 1 & 0.00                      \\
        & $10^3$ & 987 & 98.7 & 16 & 0.00                      \\
        & $10^4$ & 9719 & 97.2 & 177 & 0.01                      \\
        & $10^5$ & 94245 & 94.2 & 1560 & 0.12                      \\
        & $10^6$ & 852330 & 85.2 & 9890 & 0.76                      \\
        & $10^7$ & 6889146 & 68.9 & 39526 & 3.04                      \\
        & $10^8$ & 49044127 & 49 & 104097 & 7.99         \\


        \midrule
        \multirow{7}{*}{VAE}
        & $10^2$ & 100 & 100 & 0 & 0.00                      \\
        & $10^3$ & 1000 & 100 & 10 & 0.00                      \\
        & $10^4$ & 9996 & 99.9 & 119 & 0.01                      \\
        & $10^5$ & 99982 & 99.8 & 1369 & 0.11                      \\
        & $10^6$ & 984986 & 98.5 & 12320 & 0.95                      \\
        & $10^7$ & 9280739 & 92.8 & 82826 & 6.36                      \\
        & $10^8$ & 79478307 & 79.4 & 2811654 & 21.63         \\
    \end{tabular}
    \caption{Full evaluation for all trained models.
    All models trained on the rockyou training dataset (80\% of rockyou corpus)
    and evaluated on the test dataset (10\% of rockyou corpus).}
	\label{tab:full-results}
\end{table}

\begin{table}
    \centering
    \begin{tabular}{l|l:l:l:l}
        & \multicolumn{4}{c}{Matched \%}           \\
        \begin{tabular}[c]{@{}l@{}}
            Passwords \\Generated
        \end{tabular}      & GPT2F & GPT2S      & PassGAN & VAE  \\
        \midrule
        $10^2$              & 0.00    & 0.00    & 0.00    & 0.00      \\
        $10^3$              & 0.00    & 0.00    & 0.00    & 0.00      \\
        $10^4$              & 0.01    & 0.01    & 0.01    & 0.01      \\
        $10^5$              & 0.09    & 0.13    & 0.12    & 0.11         \\
        $10^6$              & 0.84    & 1.13    & 0.76    & 0.95      \\
        $10^7$              & 6.75    & 7.14    & 3.04    & 6.36         \\
        $10^8$              & 25.42   & 23.87   & 7.99    & 21.63
    \end{tabular}
    \caption{Comparison of matched passwords in rockyou testing dataset for each trained model.}
    \label{tab:aggregated-results}
\end{table}

\begin{table}
	\centering
	\begin{tabular}{l|l:l:l:l}
		& \multicolumn{4}{c}{Matched \%}           \\
		\begin{tabular}[c]{@{}l@{}}
			Passwords \\Generated
		\end{tabular}      & GPT2F & GPT2S      & PassGAN & VAE  \\
		\midrule
		$10^2$              & 0.00    & 0.00    & 0.00    & 0.00      \\
		$10^3$              & 0.00    & 0.00    & 0.00    & 0.00      \\
		$10^4$              & 0.01    & 0.01    & 0.02    & 0.01      \\
		$10^5$              & 0.08    & 0.15    & 0.13    & 0.11         \\
		$10^6$              & 0.53    & 1.21    & 0.70    & 0.95      \\
		$10^7$              & 4.96    & 6.4    & 2.43    & 5.34         \\
		$10^8$              & 17.63   & 17.13   & 5.85    & 15.00
	\end{tabular}
	\caption{Comparison of matched passwords in LinkedIn testing dataset for each trained model.}
	\label{tab:aggregated-results-LinkedIn}
\end{table}


==> sections_i/transformer.tex <==


In recent years the transformer architecture,
originally published in \cite{Vaswani2017} and applied to machine translation,
has become increasingly popular,
with transformer-based architectures setting new benchmarks in text generation, machine translation and other NLP tasks.

Transformers rely almost solely on self-attention to process an input text,
which considers all pairs of words in the sentence instead of the linear sequence of words.
While RNNs may lose the memory of words in the beginning of a sentence rather quickly,
transformers are able to capture long-term dependencies between words in a sentence and between sentences.

Two popular transformer-based architectures are BERT \cite{Devlin2019} and GPT2 \cite{Radford2019}.

\subsection{GPT2}

GPT2 is a transformer-based architecture developed by OpenAI,
famous for generating realistic text\footnote{\url{https://bellard.org/textsynth/}}
and for its research team not publishing the full trained model due to ethical concerns.\footnote{\url{https://openai.com/blog/better-language-models/}}
GPT2 is trained on the causal language modeling (CLM) objective, meaning given an incomplete sentence it will try to predict the next upcoming word.

The way to use this language model for text generation is completion of prompts.
Given a text prompt (eg. ``Hello my '') the model will start generating text that continues the sentence (eg. ``name is GPT2'').

In our report we train two GPT2-based models:

One model starts with the openly available GPT2 model, trained on 40GB of Internet text.
We finetune (i.e.\ continue the training of) this model with our password dataset.
We hope that the original training gives the model some background on how language is generally structured as well as a vocabulary of common words.
Finetuning on passwords should then give the model an understanding of the structures and the vocabulary of passwords and force it to generate passwords when prompted.
We call this model GPT2-Finetuned or GPT2F.

The other model only takes the architecture of GPT2 and trains a randomly initialized model from scratch.
A concern using a pretrained and finetuned model is whether the model resorts back to generating regular english text when faced with certain prompts.
A model trained from scratch will not have this problem since all text it has ever known is passwords.

\subsection{Training}

Language models like GPT2 learn from raw text.
Given a sentence it will analyse part of the sentence  and try to predict the next upcoming word.
To create a language modeling data corpus of passwords we simply take all shuffled passwords in the training dataset
and concatenate them into one long sequence of passwords, separated by whitespace.

There is no connection between two consecutive passwords.
The model should therefore learn how passwords are structured and when cued with a whitespace should generate a random password.
We train the model using an openly available implementation of GPT2.\footnote{\url{https://huggingface.co/transformers/model_doc/gpt2.html}}


